Tackling Graphical NLP problems with Graph Recurrent Networks

How to properly model graphs is a long-existing and important problem in NLP area, where several popular types of graphs are knowledge graphs, semantic graphs and dependency graphs. Comparing with other data structures, such as sequences and trees, graphs are generally more powerful in representing complex correlations among entities. For example, a knowledge graph stores real-word entities (such as "Barack_Obama" and "U.S.") and their relations (such as "live_in" and "lead_by"). Properly encoding a knowledge graph is beneficial to user applications, such as question answering and knowledge discovery. Modeling graphs is also very challenging, probably because graphs usually contain massive and cyclic relations. Recent years have witnessed the success of deep learning, especially RNN-based models, on many NLP problems. Besides, RNNs and their variations have been extensively studied on several graph problems and showed preliminary successes. Despite the successes that have been achieved, RNN-based models suffer from several major drawbacks on graphs. First, they can only consume sequential data, thus linearization is required to serialize input graphs, resulting in the loss of important structural information. Second, the serialization results are usually very long, so it takes a long time for RNNs to encode them. In this thesis, we propose a novel graph neural network, named graph recurrent network (GRN). We study our GRN model on 4 very different tasks, such as machine reading comprehension, relation extraction and machine translation. Some take undirected graphs without edge labels, while the others have directed ones with edge labels. To consider these important differences, we gradually enhance our GRN model, such as further considering edge labels and adding an RNN decoder. Carefully designed experiments show the effectiveness of GRN on all these tasks.

==> lemma.tex <==
\begin{pspicture}(0,0)(28, 2)

\pcline{|-|}(0,0)(3,0)
\pcline{|-|}(4,0)(6,0)
\rput(7.5,0){$\bigcup^*(T_1 \cup T_2)$}
\pcline{|-|}(1,1)(3,1)
\pcline{|-|}(4.5,1)(5.5,1)
\rput(7.5,1){$T_2$}
\pcline{|-|}(0,2)(2,2)
\pcline{|-|}(4,2)(6,2)
\rput(7.5,2){$T_1$}

\pcline{|-|}(10,0)(16,0)
\rput(17.5,0){$\bigcup^*(T_1 \cup T_2)$}
\pcline{|-|}(11,1)(13,1)
\pcline{|-|}(14,1)(16,1)
\rput(17.5,1){$T_2$}
\pcline{|-|}(10,2)(12,2)
\pcline{|-|}(12.5,2)(15.5,2)
\rput(10,2.4){$i$}
\rput(12,2.4){$k_1$}
\rput(11,2.4){$k_2$}
\rput(13,2.4){$j_2$}
\rput(16,2.4){$j$}
\rput(17.5,2){$T_1$}

\end{pspicture}


==> urcsmacros.tex <==
%
% urcsmacros
%
% author: Lawrence A. Crowl
% last updated: 28 April 1990
%
% BibTeX
%
\newcommand{\BibTeX}{{B\kern-.0833em{\sc ib}\kern-.1667em%
T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}
%
% SLiTeX
%
\newcommand{\SliTeX}{{\rm S\kern-.06em{\sc l\kern-.035emi}\kern-.06em
T\kern -.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%
% UNIX
%
\newcommand{\UNIX}{{\sc Unix}}
%
% trademark
%
\newcommand{\trademark}{$^{\rm TM}$}
%
% singlespacing (for use in doublespaced documents)
%
\def\doublespacefactor#1#2{%
\newenvironment{singlespace}{\baselineskip #2\baselineskip}%
{\par \baselineskip #1\baselineskip}%
\par \baselineskip #1\baselineskip}
%
% various latin abbreviations
%
\def\adhoc{{\em ad hoc}}
\def\aposteriori{{\em a posteriori}}
\def\apriori{{\em a priori}}
\def\Cf{{\em Cf.}}
\def\cf{{\em cf.}}
\def\Eg{{\em E.g.}}
\def\eg{{\em e.g.}}
\def\etal{{\em et al.}}
\def\etc{{\em etc.}}
\def\Ibid{{\em Ibid.}}
\def\ibid{{\em ibid.}}
\def\Id{{\em Id.}}
\def\id{{\em id.}}
\def\Ie{{\em I.e.}}
\def\ie{{\em i.e.}}
\def\Loccit{{\em Loc.\ cit.}}
\def\loccit{{\em loc.\ cit.}}
\def\Opcit{{\em Op.\ cit.}}
\def\opcit{{\em op.\ cit.}}
\def\qv{{\em q.v.}}
\def\Qv{{\em Q.v.}}
\def\viz{{\em viz.}}
%
% andbreak  (for breaking author lists)
%
\def\andbreak{%% \begin{tabular}
\end{tabular}\\\begin{tabular}[t]{c}%% \end{tabular}
}
%
% titlequote
%
\def\titlequote#1{\hfill
\parbox{4in}{\begin{flushright}{\small\it #1}\end{flushright}}}
%
% weekdaystring
%
% Dump the day of the week in string form.
% This macro is only valid from 1901 A.D. through 2099 A.D.
%
\def\weekdaystring#1#2#3{{% extra brace saves enclosing register state
%
% days through the end of the year
% days := current year * 365
\count10=#3%
\multiply\count10 by 365%
% leap years := year / 4
\count11=#3%
\divide\count11 by 4%
% days := days + leap years
\advance\count10 by \count11
%
% find out if the current year is a leap year
% last leap year := leap years * 4
\count12=\count11%
\multiply\count12 by 4
% years since last leap year := current year - last leap year
\count13=#3%
\advance\count13 by -\count12%
% years since last leap year equals zero when current year is a leap year
%
% subtract off those days in this month and the following months
% days = days - following days [ is leap ] [ current month ]
\ifcase#2%
\or\ifcase\count13\advance\count10 by -366% leap January
\else\advance\count10 by -365% normal January
\fi%
\or\ifcase\count13\advance\count10 by -335% leap February
\else\advance\count10 by -334% normal February
\fi%
\or\advance\count10 by -306% March
\or\advance\count10 by -275% April
\or\advance\count10 by -245% May
\or\advance\count10 by -214% June
\or\advance\count10 by -184% July
\or\advance\count10 by -153% August
\or\advance\count10 by -122% September
\or\advance\count10 by -92% October
\or\advance\count10 by -61% November
\or\advance\count10 by -31% December
\fi%
%
% update days by day of month
% days := days + current day
\advance\count10 by #1%
%
% find weekday number
% offset for initial day of the week
\advance\count10 by 5
% last monday := (current day / 7) * 7
\count14=\count10%
\divide\count14 by 7%
\multiply\count14 by 7
% weekday number := current day - last monday
\count15=\count10%
\advance\count15 by -\count14
%
% now dump out appropriate string
\ifcase\count15 Monday\or Tuesday\or Wednesday%
\or Thursday\or Friday\or Saturday\or Sunday\fi%
}}
%
% monthstring
%
% Dump the month in string form.
%
\def\monthstring#1{\ifcase#1\or January\or February\or March\or April\or May%
\or June\or July\or August\or September\or October\or November\or December\fi}
%
% dateWDMY
%
% Redefine \today as "weekdaystring daynumber monthstring yearnumber" format.
%
\def\dateWDMY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\number\day\space\monthstring{\month}\space\number\year}}
%
% dateDMY
%
% Redefine \today as "daynumber monthstring yearnumber" format.
%
\def\dateDMY{\def\today{\number\day\space\monthstring{\month}%
\space\number\year}}
%
% dateWMDY
%
% Redefine \today as "weekdaystring monthstring daynumber, yearnumber" format.
%
\def\dateWMDY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\monthstring{\month}\space\number\day,\space\number\year}}
%
% dateMDY
%
% Redefine \today as "monthstring daynumber, yearnumber" format.
%
\def\dateMDY{\def\today{\monthstring{\month}\space\number\day,%
\space\number\year}}
%
% dateMY
%
% Redefine \today as "monthstring yearnumber" format.
%
\def\dateMY{\def\today{\monthstring{\month}\space\number\year}}
%
% dateY
%
% Redefine \today as "yearnumber" format.
%
\def\dateY{\def\today{\number\year}}

